Quantum Information Driven Ansatz (QIDA): shallow-depth empirical quantum circuits from Quantum Chemistry

Hardware-efficient empirical variational ans\"atze for Variational Quantum Eigensolver simulations of Quantum Chemistry suffer from the lack of a direct connection to classical Quantum Chemistry methods. In the present work, we propose a method to fill this gap by introducing a new approach for constructing variational quantum circuits, leveraging quantum mutual information associated with classical Quantum Chemistry states to design simple yet effective heuristic ans\"atze with a topology that reflects the correlations of the molecular system. As first step, Quantum Chemistry calculations, such as M{\o}ller-Plesset (MP2) perturbation theory, firstly provide an approximate Natural Orbitals basis, which has been recently shown to be the best candidate one-electron basis for developing compact empirical wavefunctions (Ratini, et al 2023). Secondly, throughout the evaluation of quantum mutual information matrices, they provide information about the main correlations between qubits of the quantum circuit, enabling the development of a direct design of entangling blocks for the circuit. The resulting ansatz is then utilized with a Variational Quantum Eigensolver (VQE) to obtain a short depth variational groundstate of the electronic Hamiltonian. To validate our approach, we perform a comprehensive statistical analysis by simulations over various molecular systems ($H_2, LiH, H_2O$) and apply it to the more complex $NH_3$ molecule. The reported results demonstrate that the proposed methodology gives rise to highly effective ans\"atze, surpassing the standard empirical ladder-entangler ansatz in performance. Overall, our approach can be used as effective state preparation providing a promising route for designing efficient variational quantum circuits for large molecular systems.

==> tabelle_test.tex <==
\begin{table}[h]
       \centering
       \begin{tblr}{hlines, vlines, colspec={cccccc}}
       \SetCell[c=1,r=3]{} molecule & \SetCell[c=1,r=3]{} \mu & \SetCell[c=1,r=3]{} janitor sequence & \SetCell[c=3,r=1]{} maximal quantum mutual information \\
       & & & \SetCell[c=2,r=1]{} HFO & NO \\
       & & & FCI & FCI & MP2 \\
       $H_{2}$ & 0.5 & \{[0, 1], [0, 5], [4, 5], [0, 4], [1, 5], [1, 4]\} & 0.0539 & 0.0542 & 0.0539 \\
       $LiH$ & 0.5 & \{[0, 4], [0, 5], [0, 9],[4, 5],[4, 9], [5, 9]\} & 0.0698 & 0.0780 & 0.0705  \\
       \SetCell[c=1,r=4]{} $H_{2}O$ & \SetCell[c=1,r=2]{} 0.5 & \SetCell[c=1,r=2]{}
           \{[1, 5], [1, 7], [ 1, 11], [2, 4], [2, 8], [ 2, 10], \par 
           [ 4, 10], [5, 7], [ 5, 11], [ 7, 11], [ 8, 10]\}
       & \SetCell[c=1,r=4]{} 0.0277 & \SetCell[c=1,r=4]{} 0.0277 & \SetCell[c=1,r=4]{} 0.0277 \\
       & \SetCell[c=1,r=2]{} 0.7 & \SetCell[c=1,r=2]{} \{[1, 5], [1, 7], [ 1, 11], [2, 4],[ 4, 10], \par
       [5, 7], [ 5, 11], [ 7, 11], [ 8, 10]\} & & & \\
       %& 0.5 reduced &  \{[1, 5], [2, 4],[ 4, 8], [5, 7], [ 7, 11], [ 8, 10]\} & & & \\
       \end{tblr}
\caption{Summary of data of the systems under analysis and computational details. The maximal mutual information values represent the normalization constants of the $I$ maps shown in figure}      
\end{table}


\begin{table*}[h]
\centering
\newcommand{\minitab}[2][l]{\begin{tabular}#1 #2\end{tabular}}
\begin{tabular}{c|c|c|c|c|c }
\hline
\hline
molecule & $\mu$ & janitor sequence & \multicolumn{3}{c}{ maximal quantum mutual information } \\
& & & HFO & \multicolumn{2}{c}{ NO } \\
\hline
$H_{2}$ & 0.5 & \{[0, 1], [0, 5], [4, 5], [0, 4], [1, 5], [1, 4]\} & 0.0539 & 0.0542 & 0.0539 \\
\hline
$LiH$ & 0.5 & \{[0, 4], [0, 5], [0, 9],[4, 5],[4, 9], [5, 9]\} & 0.0698 & 0.0780 & 0.0705  \\
\hline
$H_{2}O$ & 0.5 & \minitab[c]{\{[1, 5], [1, 7], [ 1, 11], [2, 4], [2, 8], [ 2, 10],\\ 
[4, 8], [ 4, 10], [5, 7], [ 5, 11], [ 7, 11], [ 8, 10]\}} & 0.0277 & 0.0277 & 0.0277 \\

\hline
$NH_{3}$ & 0.5 & \{[0,4], [1,5], [2,6], [4,7], [5,8]\} & 0.0277 & 0.02516  & 0.02517 \\


%\{[1, 5], [1, 7], [ 1, 11], [2, 4], [2, 8], [ 2, 10], \\
%[4, 8], [ 4, 10], [5, 7], [ 5, 11], [ 7, 11], [ 8, 10]\}\\
%   &   & 0.7  & \{[1, 5], [1, 7], [ 1, 11], [2, 4],[ 4, 10], \\
%[5, 7], [ 5, 11], [ 7, 11], [ 8, 10]\}\\
%&&&\\
%   &   & 0.5 \textit{reduced}  & \{[1,5], [2,4], [4,8], [5,7], [7,11], [8,10]\}  & 0.0277 & 0.0277 & 0.0277   \\
%& \textbf{H} : 0.757, 0.586, .0&&&&&& \\
% & \textbf{H} : -0.757, 0.586, .0&&&&&& \\
%  \textbf{$NH_{3}$}  & \textbf{N} : .0, .0, 0.1211& sto-3G & Yes  & 14  & 0.0277 & 0.02516  & 0.02517    \\
% & \textbf{H} : .0, 0.9306, -0.2826&&&&&& \\
% & \textbf{H} : 0.8059, -0.4653, -0.2826&&&&&& \\
% & \textbf{H} :  -0.8059, -0.4653, -0.2826&&&&&& \\
\hline
\hline
\end{tabular}
\caption{Summary of data of the systems under analysis and computational details. The maximal mutual information values represent the normalization constants of the $I$ maps shown in figure \ref{fig:maps}.}
\label{tab: systems}
\end{table*}
